Multi-agent cooperation through learning-aware policy gradients

Self-interested individuals often fail to cooperate, posing a fundamental challenge for multi-agent learning. How can we achieve cooperation among self-interested, independent learning agents? Promising recent work has shown that in certain tasks cooperation can be established between learning-aware agents who model the learning dynamics of each other. Here, we present the first unbiased, higher-derivative-free policy gradient algorithm for learning-aware reinforcement learning, which takes into account that other agents are themselves learning through trial and error based on multiple noisy trials. We then leverage efficient sequence models to condition behavior on long observation histories that contain traces of the learning dynamics of other agents. Training long-context policies with our algorithm leads to cooperative behavior and high returns on standard social dilemmas, including a challenging environment where temporally-extended action coordination is required. Finally, we derive from the iterated prisoner's dilemma a novel explanation for how and when cooperation arises among self-interested learning-aware agents.

==> blobs.tex <==

\begin{comment}
Contributions:
- achieving cooperation in social dilemma's with purely selfish objectives
- policy gradient algorithm for scalable opponent shaping
- higher-derivate-free LOLA estimator
- Detailed analysis of when and why cooperation arises through selfish objectives with co-player learning awareness.

Abstract
- intro sentence that RL in general sum games exhibiting social dilemmas defect
- Here, we show that by incorporating information on the learning behavior of co-players in the agent updates, we can achieve cooperation in sequential social dilemma's with temporal extended actions. 
- We achieve this in a simple and scalable way by training the agents on multiple concatenated episodes, encompassing multiple co-player updates. We derive an unbiased policy gradient method for the realistic setting where co-players use trajectory batches to update their parameters, making our approach significantly more sample-efficient compared to previous approaches based on evolutionary search. 
- As a special case of our method, we obtain a simple higher-derivative-free estimator of the well-known 'Learning with opponent learning awareness' update \mref, which leads to more robust training. 
- We provide a detailed analysis of when and why cooperation arises through selfihs objectives with co-player learning awareness. 
\end{comment}

% COPY OF PREVIOUS ABSTRACT STATE
%Self-interested individuals often fail to cooperate. This simple observation has profound implications for multi-agent machine learning, where learning by independent reward maximization is typically more efficient, easier to implement, or the only available option. How can we achieve cooperation among self-interested, independent learning agents? Promising recent work has shown that in certain tasks cooperation can be established between agents that model the learning dynamics of each other, an approach referred to as `learning-aware'. Here, we present the first unbiased, higher-derivative-free policy gradient algorithm for learning-aware reinforcement learning, which takes into account that other agents are themselves learning through trial and error based on multiple noisy trials. We then leverage efficient sequence models to condition behavior on long observation histories that contain traces of the learning dynamics of other agents. When trained with our algorithm, the resulting policies develop cooperative behavior and collect high returns on standard social dilemmas, including a previously unsolved environment where temporally-extended action coordination is required. Finally, by analyzing the iterated prisoner's dilemma, we uncover a novel explanation for how and when cooperation arises among self-interested learning-aware agents.


% selectively cooperating with equally-capable agents and extorting lesser-capable ones.

%As a special case of our method, we obtain a higher-derivative-free estimator of the well-known `learning with opponent learning awareness' algorithm. Finally, we analyze the classical iterated prisoner's dilemma, and uncover a novel explanation for how cooperation may arise among self-interested, learning-aware agents.

%Self-interested individuals often fail to cooperate. This simple observation has profound implications for multi-agent machine learning, where learning by independent reward maximization is typically more efficient, easier to implement, or the only available option. How can we achieve cooperation among self-interested, independent learning agents? Promising recent work has shown that in certain tasks cooperation can be established between agents that model the learning dynamics of each other, an approach referred to as `learning-aware'. Here, we present the first unbiased, higher-derivative-free policy gradient algorithm for learning-aware reinforcement learning, which takes into account that other agents are themselves learning through trial and error based on multiple noisy trials. We incorporate information on the  long-context policies that condition behavior on long observation histories containing traces of the learning dynamics of other agents. and find that the high returns on social dilemmas

\begin{comment}
\begin{abstract}
[intro sentence that MARL is gaining on importance, but that agents trained on individual (selfish) objectives in general sum games exhibiting social dilemmas converge to poor equilibria (defecting)]
Here, we show that by incorporating information on the learning behavior of co-players in agent updates, we can achieve cooperation in sequential social dilemma's with temporal extended actions. 
We achieve this in a simple and scalable way by training the agents on multiple concatenated episodes, encompassing multiple co-player updates. We derive an unbiased policy gradient method for the realistic setting where co-players use trajectory batches to update their parameters, making our approach significantly more sample-efficient compared to previous approaches based on evolutionary search. 
As a special case of our method, we obtain a simple higher-derivative-free estimator of the well-known `Learning with opponent learning awareness' update \mref, which leads to more robust training. 
We provide a detailed analysis of when and why cooperation arises through selfish objectives with co-player learning awareness. We show that our method scales beyond iterated matrix games. 
\end{abstract}
\end{comment}



\paragraph{Relationship to prior work.} \mrefa{Placeholder, needs to be entirely rewritten} Shaper and M-FOS \mref meet this halfway, having a distinct policy for each trajectory in the minibatch, i.e. have a factorized action distribution instead of a joint one, but sharing information of the ongoing long histories in the batch at each inner episode boundary, through averaging the sequence model's activations along the batch dimension, or providing a conditioning the policies based on the full batch of long histories, respectively. The Shaper \mref and Good Shepherd \mref methods consider this flattened co-player shaping problem, with a policy $\pi^i$ conditioned on the long history $h^i_t$ and inner history $x_{t,m}^i$, respectively, using evolutionary strategies. 



Notable differences with M-FOS, Shaper
\begin{itemize}
    \item M-FOS and Shaper's policies are factorized, but relies on cross-batch information. At timestep $t$ of the $m$-th inner episode, Shaper's policy depends on the inner episode history, as well as the batched long history up to the beginning of the current inner episode, i.e.  $\pi(a^{i,b}_{mT+t}|h_{mT:mT+t}^{i,b}, \bar{h}_{1:mT}^i)$. As for M-FOS, it depends on the current inner episode and previous batched inner episode, $\pi(a^{i,b}_{mT+t}|h_{mT:mT+t}^{i,b}, \bar{h}_{(m-1)T:mT}^i)$. In contrast, we consider policy of the form $\pi(a^{i,b}_{mT+t}|h_{1:mT+t}^{i,b})$.
    \item To achieve this, M-FOS has a specialized bilevel architecture: the meta policy takes as input the previous batched episode, and produces the parameter or a conditioning vector from $\pi^{meta}(z^i_m | \bar{h}_{(m-1)T:mT}^i)$ for the inner policy, which then acts in the environment following $\pi(a^{i,b}_{mT+t}|h_{mT:mT+t}^{i,b}, z_m^i)$. This is an architecture specialized for playing against naive opponents in a batched setting, but in general is awkward when playing against e.g. other meta agents. On the other hand, because of our flattened formulation of the MDP, we can simply use any general purpose sequence models. As for Shaper, while it also has a "flat" architecture similarly to us, additional tricks are required to propagate the cross-batch information. 
    \item TLDR: we simplify the parametrization such that it is inner-batch agnostic, and use a "clean" policy gradient so that the model learns to behave nicely whether it is in the batch or unbatched setting.
\end{itemize}


\begin{comment}
To formalize this approach, let us consider first a simplified setting where co-players update their policies based on the experience of a single inner episode $x_T^{-i}$. This neglects the fact that RL agents require in practice multiple inner episodes (`minibatches') to make significant progress; we return to this important point below. We can then flatten the meta and inner levels by concatenating $M$ inner episodes $x_{T,m}$ into a long history $h_{MT} = \{x_{T,m}\}_{m=0}^M$. The naive learner co-players have policies $\pi\mi$ that only take the history of the current inner episode into account, whereas the learning-aware agent has a policy $\pi^i(a_t \mid h_t;\phi^i)$ that takes the long history $h$ into account up until the current timestep $t$. In this setup, its sequence model parameters $\phi^i$ now take on the role of both the inner policy parameters and the meta-policy parameters: using the current inner episode history $x_{t,m}^i$, the model simulates an inner policy, whereas when using the long history $h_t^i$ of the previous inner episodes, it can simulate parameter updates $\phi^i_m$, by changing the internal state of the sequence model. Furthermore, using in-context learning, the sequence model can infer the current parameters $\phi\mi$ of the co-players, thereby giving it full access to the meta state $(\phi^i_m, \phimi_m)$. Taken together, this leads to the following single-level co-player shaping problem:
\begin{align}\label{eqn:flat_shaping_problem}
    \max_{\phi^i}\bbE_{\bar{P}_i(\phimi_0)}\expect{\bar{P}^{\pi^i}}{\sum_{t=t_{\mathrm{start}}}^{MT} R^i_t}
\end{align}
When co-players update their policies based on multiple inner episodes, the flattened co-player shaping problem becomes more intricate, a challenge that we address in Section \ref{sec:coala}.
\end{comment}



\begin{comment}
\begin{itemize}
    \item Partially observable stochastic games
    \item Selfish objectives
    \item Non-stationarity and equilibrium selection
    \item Opponent shaping: raising to the meta-level to remove the non-stationarity. Explain this leads to single agent policy. Explain optimal control problem, and flattening to single level. Explain different types of memory and why they are necessary (inner episode policy and inferring parameters of others and having a different policy each inner episode)
    \item What happens when two shapers play against each other?
    \item What happens when other player uses inner episode batches to update its policy?
\end{itemize}

\textbf{Notation.} Let us take $P(h_{t+1:T} \mid h_t, a_t; \theta^i, \theta^{-i})$ the distribution over future histories $h_{t+1:T}$ starting from history $h_t$ and taking action $a_t$, unrolling the main player policy $\theta^i$ and co-player policies $\theta^{-i}$. We assume for now that all players observe the shared histories $h_t$, i.e. that we do not have different player-specific histories $h^i_t$. We use the notation $\{h^b\}_{b=1}^B \sim P(h \mid h_t, a_t; \theta^i, \theta^{-i})$ to indicate drawing a batch of $B$ histories drawn from the distribution $P$. When the naive learner updates on a minibatch of inner-episodes, the trajectories consisting of multiple inner episodes become dependent on each other. We use shorthand $x_t = \{h^b_t\}_{b=1}^B$. All trajectories in the minibatch are sampled independently from each other.
\end{comment}




\begin{comment}
Relevance of multi-agent RL: AI applications in the world are becoming more and more multiagent (self-driving cars, personalized assistants, ...). In settings with repeated interactions + learning, it becomes crucial to ensure that learning progresses towards beneficial outcomes.

Setting: General sum games with decentralized training: 
\begin{itemize}
\item agents have individual goals
\item require both cooperation and competition to achieve good solutions
\item Agents do not share privileged information during training
\item such settings give rise to social dilemmas: short-sighted incentives to defect, while mutual defection leaves everyone worse off compared to mutual cooperation. 
\end{itemize}

While good results in multi-agent RL have been achieved in the fully cooperative or zero-sum setting, these algorithmic advances have not translated towards the general sum setting. IPD example: independent RL leads to mutual defection, while much more beneficial equilibria exist.

Why? Main challenges of multi-agent RL where we focus on:
\begin{itemize}
\item Environment Non-stationarity due to learning of co-players (Papoudakis 2019 review)
\item Equilibrium selection: In realistic long-horizon games, often infinitely many Nash Equilibria (Folk theorems).
\item RL algorithms don't take the influence of actions on the learning of other agents into account, hence naively assume they can 'get away with defecting', often leading to defecting equilibria.
\end{itemize}
Solving social dilemmas with decentralized RL is an open problem!
Two main strategies: reward shaping (or more general changing of the environment) and endowing agents with co-player learning awareness.

Quick summary paragraph on reward shaping and environment shaping side
\begin{itemize}
    \item Sequential social dilemma's (Leibo et al. 2017) (iterated matrix games is not all you need)
    \item pro-social reward shaping (whole 'solving sequential social dilemma's' section in the paper doc)
    \item intrinsic reward for influencing others (Jaques et al. 2019)
\end{itemize}

Algorithmic side: co-player learning awareness (or opponent shaping / co-player shaping).
\begin{itemize}
    \item Leverage information about the learning dynamics of other agents: (i) anticipate environment non-stationarity; (ii) empirically observed that this leads to better equilibria, however this is not yet well understood why. 
    \item LOLA: backpropagates gradient through anticipated opponent update to influence the learning one step ahead. First to show cooperation emerge in IPD through these adjusted policy gradients
    \item Later generalized by MAML-type approach that include: (i) multiple look-ahead steps, (ii) anticipate also your own policy updates by naive gradient updates, (iii) consider distribution over opponents (i.e. trains against many different opponents instead of a single one as in LOLA). (Kim et al. 2021, (Al-Shedivat et al. 2018)Learning to Exploit (L2E) (Wu et al., 2021) 
    \item Inconsistent assumption on the co-player learning when doing self-play or co-players with co-player learning awareness. COLA (willi et al 2022) and Meta Value (Cooijmans et al. 2023) address this issue by introducing consistency relations and solve these over the whole parameter space by optimizing a parametric model of the updates.
    \item M-FOS, Shaper, Good Shepard ( Balaguer et al. 2022) Lili (Xie et al. 2020) take a general model-free approach to opponent shaping making no assumptions on the co-player learning dynamics, only that they can simulate many learning trajectories to estimate meta gradients.
\end{itemize}

Importance of 'bitter-lesson proof' algorithms. Shaper takes a first step into this direction by flattening the meta level and optimizing a sequence model policy over concatenated episodes. However, no policy gradient algorithm exists to date that can handle this setting (minibatch issue), as Shaper uses genertic algortihms. Furthermore, this flattened setting has only been tested the pure shaping setting, not whether cooperation arises when playing against equally capable co-players. 

In general little mechanistic understanding of why mixing shaping scenarios with training against equally capable agents results in cooperative behavior with those capable agents. 

Contributions
\begin{itemize}
    \item PG algorithm for scalable opponent shaping via concatenated episode sequence modelling
    \item higher-derivative-free LOLA estimator
    \item Mechanistic understanding why opponent awareness leads to cooperation
    \item detailed experiments
\end{itemize}

\end{comment}


\begin{comment}
\textbf{[New structure]}

\textbf{Incorporating co-player learning awareness into multi-agent setting with equally capable agents.} Merge 3.2 with opening paragraph of this section and compress

\textbf{Why does naive independent learning lead to bad outcomes?} Compress section 3.1, and introduce the iterated prisoner's dilemma and experimental setup for the analytical results (assuming social dilemmas have been introduced in the introduction or background, otherwise we need to do it here as well). First empirical result on analytical IPD (panel in main figure of section 3): best response against a randomly initialized policy leads to unconditional defection with high probability. 
\end{comment}



\begin{comment}
\textbf{[old structure]}


The co-player shaping problems (\ref{eqn:shaping_problem}-\ref{eqn:flat_shaping_problem}) consider an asymmetric setting where the ego agent $i$ has co-player learning awareness, whereas all other agents are naive learners. However, ultimately we are interested in deploying these algorithms in situations with equally-capable co-players. Empirical results indicate that multi-agent settings where all players have co-player learning awareness can lead to cooperative behavior, a striking result with to-date no clear understanding on why this cooperation emerges. Endowing co-players with co-player learning awareness removes many of the convenient properties of the co-player shaping problems (\ref{eqn:shaping_problem}-\ref{eqn:flat_shaping_problem}): (i) in LOLA and Meta-MAPG \mref this leads to an inconsistency of assuming that co-players are naive learners, while in reality they are co-player learning aware \mrefa{Willi et al. 2022 COLA}, and (ii) in M-FOS, Shaper and Meta Value \mref, it changes the stationary single-agent meta-level of the shaping problem into a multi-agent setting, introducing again the non-stationarity and equilibrium selection problems. Understanding when and why cooperative behavior emerges in this setting of equally capable players is an important open question. In this section, we provide a detailed hypothesis for the emergence of cooperation, which we validate here empirically on the discounted infinitely iterated prisoners dilemma accessing the analytical gradients, and later in more realistic reinforcement learning settings in Section \ref{sec:experiments}.

\subsection{Why does naive independent learning lead to bad outcomes?}

We start by analyzing why multi-agent social dilemmas with independent learners without co-player learning awareness lead with high probability to low-reward outcomes for all players. As a guiding example, we consider the infinitely iterated prisoners dilemma, a matrix game with two possible actions for each agent: cooperate (C) and defect (D), played with two agents over infinitely many rounds. The reward structure of the game (see Table \mref) makes it a social dilemma: considering a single timestep, defecting results in a higher reward for the agent, independent of the action of its co-player; considering the (infinite) future however, it is better to play a policy leading to mutual cooperation, compared to a policy leading to mutual defection. There exist infinitely many nash equilibria for this setting \mref, leading to both mutual defection outcomes or mutual cooperation outcomes. While mutual cooperation outcomes are preferred to both agents compared to mutual defection outcomes, independent reinforcement learning with the expected individual return as objective leads to mutually defecting outcomes for most policy initializations. 

The central problem with independent learning is that from a single agent's perspective, the environment is non-stationary as the co-players are also learning, whereas the RL updates only consider the current episode and hence do not take into account the influence of the agent's actions on this non-stationarity. As the co-player policies are considered fixed during the RL update, the agents do not receive learning feedback that (i) unilateral defection causes the co-players to update their policies towards more defection, leading to lower future rewards, and (ii) punishing co-players for defection and rewarding them for cooperation causes the co-players to update their policies towards more cooperation, leading to higher future rewards. Randomly initialized policies are unstructured with high probability, i.e. they do not have coherent strategies to punish defection from co-players or reward cooperation. Hence, in the beginning of training, the agents get clear learning feedback from the independent RL algorithms that they can 'get away with defection', and hence start to defect more and more, ultimately leading to a mutual defection equilibrium. While this explanation is most easily applicable to iterated matrix games with a cooperate and defect action, our main arguments are applicable to any general sum environments where agents can deploy both 'asocial' defect strategies, or 'prosocial' cooperate strategies.

Co-player learning awareness introduces the missing ingredient of providing learning feedback on the influence of the agent's actions on the non-stationarity of the environment, i.e. the co-player's learning updates. Now the question remains how exactly this co-player learning awareness leads to cooperation. Before we can state our main hypothesis, however, we need to discuss how to make the co-player shaping problem compatible with multi-agent systems of equally capable agents. 

\subsection{Incorporating co-player learning awareness into multi-agent setting with equally capable agents}
We focus our exposition on how to incorporate co-player learning awareness mainly on the flattened shaping setting of Eq. \ref{eqn:flat_shaping_problem} with model-free RL agents, and later indicate how to generalize it towards other co-player learning awareness methods. In this setting, what distinguishes co-agent learning aware agents (COALA agents) from naive learners is that they take the long histories $h$ into account in their policy updates, compared to naive learners which learn on a faster timescale considering inner episode histories $x_m$. When COALA agents play against each other, they all learn on the same timescale, but now considering long histories instead of inner-episode histories. Hence, this is again the multi-agent setting with independent learning, suffering from the non-stationarity problem and equilibrium selection problem, and will not lead to cooperative outcomes in general.

To infuse co-player learning awareness into this setting, we make a distinction between \textit{agents} and \textit{players}. We introduce a \textit{population} of an arbitrary amount of agents, consisting of a mix of COALA agents taking long horizons into account in their learning, and naive learning agents using inner-episode histories $x_m$ in their learning updates. We then simulate many multi-agent games of $n$ players, by selecting with replacement $n$ agents out of the population and letting them play the n-player POSG (allowing for self-play). As COALA agents now play against both other COALA agents and naive learners, there is a possibility of transferring the co-player learning awareness gained from playing against naive learners towards COALA co-players. For this transfer to take place reliably, the COALA agent policies should either (i) have only limited information about the agent identity of their co-players, such that at the beginning of the game, they play similar strategies against both naive learners and COALA agents, or (ii) have a deep network policy that shares representations when playing against naive learners or COALA agents. Furthermore, the naive learners should use similar goal-oriented learning strategies compared to the COALA agents, although we argue that a strict equality of learning strategies is not required for the emergence of cooperation to appear, as we will become clear in the next section. 

M-FOS \mref adopts a special setting of this population-based approach, by having one M-FOS agent that plays both against itself, as well as randomly initialized naive learners. LOLA \mref also adopts a special case of our population-based setting, by having a population of two LOLA agents and two naive learners, and only play against a naive learner that is initialized with the current parameters of the other LOLA agent. 

In general, the core principle of our population-based approach is to play both against COALA agents that learn on the same timescale, as well as other naive learners learning on a faster timescale, such that co-player learning feedback is present in the independent RL updates. Note that need not be a real separation of capabilities between `smart' agents and `easy-to-manipulate' agents in a population, as the naive learners can be purely imaginative. By modeling the other agents and their learning algorithm based on past experience, model-based COALA agents can unroll multiple learning episodes in imagination, effectively simulating co-players learning on a faster timescale to solve the co-player shaping problem \eqref{eqn:flat_shaping_problem} within imagination.


\subsection{The cooperation hypothesis}
Finally we are ready to put the pieces of the puzzle together. Our main hypothesis follows the following line of arguments:
\begin{enumerate}
    \item From a selfish individual perspective, regardless of the ego-agent's current policy, it always leads to higher rewards in social dilemmas if the co-players cooperate more.
    \item The shaping problem is a single-agent RL problem, and hence can be solved to high expected individual return, beyond the expected return provided by mutual defection. Shaping naive learners towards higher selfish return means shaping them to cooperate more. This requires a shaping policy that provides the naive learner with higher returns when cooperating compared to defecting.
    \item Such shaping policies punish defection and/or reward cooperation, similar to the tit-for-tat strategy in IPD. However, the shaper policy does not need to be 'fair', it can adopt a strategy that still punishes defection and/or rewards cooperation, while ensuring a larger return for itself compared to the return of the co-players, similar to Zero-Determinant Extortion strategies in IPD \mref. Indeed, the shaper objectives (\ref{eqn:shaping_problem}-\ref{eqn:shaping_problem}) motivate the shaper policy to move beyond fair tit-for-tat-style policies and extort the naive learner, which is confirmed empirically by M-FOS \mref.
    \item Now the question remains what happens when shaper policies play against other shaper policies in the population. Fair tit-for-tat-style policies form a Nash Equilibrium when played against each other, and are hence consolidated when these policies play against each other. Unfair extortion policies do not form a Nash Equilibrium, as the best response against an extortion policy is to mostly cooperate \mref, whereas extortion policies themselves only cooperate the bare minimum. As extortion-style policies shape the co-player to cooperate more, when two extortion-style policies face each other, independent RL will result in a policy gradient pointing towards a more cooperative policy. This will push the extortion-style shaping policies towards more fair tit-for-tat-style shaping policies. For the IPD, we show this analytically (TODO) in Theorem \mref, and empirically in Figure \mref.
\end{enumerate}

In conclusion, having a population of agents where agents play both against other co-player learning aware agents, as well as (simulated/imagined) naive learners, provides the necessary learning feedback on the influence of ones own actions on the learning of co-players, resulting in learning dynamics towards fair tit-for-tat-style shaping policies. Note that it is crucial that agents do not only play against naive learners, but also against other equally-capable agents, such that extortion-like policies are converted into more fair tit-for-tat-style policies. Hence, LOLA-type algorithms which base their updates solely on (imagined) naive learners provide updates that push towards more extortion-type policies that have problems with convergence, which aligns with the findings of \mrefa{Stable opponent shaping}

\end{comment}

\begin{comment}

\begin{itemize}
    \item Paragraph explaining why we care about shaping: (i) general 'learning with opponent learning awareness' setting. (ii) makes it possible to learn to escape bad equilibria, as it is a single-agent setting.
    \item Why is it relevant to realistic settings with all 'capable agents' and no easy-to-manipulate naive agents? (i) taking learning of other capable agents into account shows a way out of bad defection equilibria (the hope on a better future), in contrast to naive single-agent RL which always assumes the environment is fixed and not influencable. (ii) Easy to justify in a model-based setting, modeling the learning of the opponent.
    \item Explain population-based setting
    \item Explain main hypothesis
    \item Why do we care about shaper architecture and not the explicit meta levels etc? (i) bitter-lesson-proof: leverage highly capable sequence models. (ii) compatible with out-of-the-box RL algorithms (with minibatchsize=1)
    \item Main shortcoming: how to conceptualize and train it with PG if co-player uses minibatches?
\end{itemize}
\subsection{Population-based training with co-player learning awareness}
\begin{itemize}
    \item Setup: a mix of main agents and naive learners
    \item For complex environments, not realistic to put full learning trajectory of a naive learner in context, hence good initializations needed. We can achieve this by putting a 'naive learner wrapper' around previous checkpoints of main agent policies, as anyway all policies (main and naive) are sequence models. 
    \item Intuition on why this leads to cooperation: (i) against naive is single-agent RL problem which can be fully solved; (ii) The single-agent learning trajectory will go through a cooperation phase; (iii) at this phase, main agents cooperate against naive ones, and will also learn to cooperate against other main ones; (iv) later on, main will start exploiting naive learners, but cannot exploit main ones, so will keep cooperating against main ones. 
    \item This hypothesis will be tested and shown in detail in the experimental section
\end{itemize}t

\end{comment}



